Blowup analysis of a hysteresis model based upon singular perturbations

In this paper, we provide a geometric analysis of a new hysteresis model that is based upon singular perturbations. Here hysteresis refers to a type of regularization of piecewise smooth differential equations where the past of a trajectory, in a small neighborhood of the discontinuity set, determines the vector-field at present. In fact, in the limit where the neighborhood of the discontinuity {vanishes}, hysteresis converges in an appropriate sense to Filippov's sliding vector-field. Recently {(2022)}, however, {Bonet and Seara} showed that hysteresis, in contrast to regularization through smoothing, leads to chaos in the regularization of grazing bifurcations, even in two dimensions. The hysteresis model we analyze in the present paper -- which was developed by {Bonet et al in a paper from 2017} as an attempt to unify different regularizations of piecewise smooth systems -- involves two singular perturbation parameters and includes a combination of slow-fast and nonsmooth effects. The description of this model is therefore -- from the perspective of singular perturbation theory -- challenging, even in two dimensions. Using blowup as our main technical tool, we prove existence of an invariant cylinder carrying fast dynamics in the azimuthal direction and a slow drift in the axial direction. We find that the slow drift is given by Filippov's sliding {vector-field} to leading order. Moreover, in the case of grazing, we identify two important parameter regimes that relate the model to smoothing (through a saddle-node bifurcation of limit cycles) and hysteresis (through chaotic dynamics, due to a folded saddle and a novel return mechanism).

==> reply.tex <==

\section*{Reviewer reply}

% Point-by-point responses to specific issues raised by the referee are given below. 
% Section \ref{sec:3} enumerates a small number of additional (minor) corrections to the manuscript.

% \section*{Reviewer \# 1 feedback and reply}
% \textbf{Feedback:} It has been a pleasure to read the survey article by K.U. Kristiansen, which I find well written and
% very instructive. 
% 
% \
% 
% 
% \textbf{Response:} We thank the referee for the positive assessment.



% \subsection*{Reviewer remarks and point-by-point response}

I thank both referees for their positive assessment of the manuscript. 

I am particularly happy about the feedback from referee \#2 regarding my effort to explain things in detail throughout. 

The reviewers' specific comments/remarks are enumerated below in italics. Each is followed by a response, with explicit reference to any changes/revisions to the manuscript accordingly. Specific changes described herein are indicated in red in the (revised) manuscript. (Other changes to the manuscript that do not relate to the referees' comments are in blue. )

\begin{remark}
 Please notice that I can see a path-name (C:/Users/...) in the shared dvi-file from referee \# 2. This could be used to identify the referee. 
\end{remark}
% (NB! 


 \section*{Reviewer \# 1 feedback and reply}

\begin{enumerate}[series=rev1]
	\item \textit{page 5, line 11: Put the references in an increasing order.
}
\end{enumerate}

\

\textbf{Response:} Thanks for spotting this. Corrected. 

\




\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 6, line 10: ``by Fenichel’s theory ...''. Put the page of cite the
number of the theorem in [7].
}
\end{enumerate}

\

\textbf{Response:} I've included a reference to \cite[Theorem 2]{jones_1995} and expanded the proof. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 7, Equation 13: How was obtained this change of variables ? I
saw why this will be good, but how it can be obtained ? for the literature,
I believe that it is important this consideration. Also page 11 Equation 19.
Also page 23 Equation 46. Also page 24 lines 6-8 and Equation 49. Also
page 35 Equation 62.
}
\end{enumerate}

\

\textbf{Response:} I agree that this is important. However, displaying \eqref{213} on p. 7 is in antipication of the blowup approach. In particular, I write: ``Our blowup approach \response{(see \secref{lem:P22})} will motivate coordinates, including ... \eqref{213}'', so the additional explaination that the referee is looking for is (hopefully) available in the new section \secref{diffblowup}. I have also included further discussion on the pages 23 and 35. The equations that the referee refer to on pp. 11 and 24 are charts. I believe the manuscript reflects this in an adequate way (see also the new section on charts, \secref{newDirectional}). 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{please revise the title of the reference [25].
}
\end{enumerate}

\

\textbf{Response:} Thanks for spotting this. The title is corrected.

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 20: In my opinion, the proof of the Lemma 3.5 must be detailed.
}
\end{enumerate}

\

\textbf{Response:} Thanks. I agree and I've therefore included a proof as suggested.

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 20: In my opinion, the proof of the Lemma 3.5 must be detailed.
6 - page 21, line 14: Please, give more details about the sentence: ”the
set Q21 acts like a fold point”.
}
\end{enumerate}

\

\textbf{Response:} Thanks. That is a good point. I've added more text to explain the meaning. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 21, last line: Why the blow up is not applied to Q21 at this
moment ?Also page 22, line 13.
}
\end{enumerate}

\

\textbf{Response:} The reason for not including the blowup at this stage is that the diagram in \figref{pws_hysteresis_final0} does not require this. In particular, it is my belief that the reader can understand the overall dynamics without the technical details involved in blowing up $Q$. I hope that the reply to the previous issue raised by the referee makes this point clearer. I have therefore deliberately chosen to push the blowup into \secref{lem:P22} where it is needed for the rigorous proof of \lemmaref{lem:P22}. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 31 Figure 14: Maybe I lost the proof, but why the point connecting the blue line (up stairs) and the purple curve is hyperbolic and it is
not must be considered a blow up on it ?
}
\end{enumerate}

\

\textbf{Response:} I guess the referee means \figref{pws_hysteresis_final}? This figure is after blowup of $Q$. In \figref{pws_hysteresis_final0}, the end-point that the referee is pointing to is fully nonhyperbolic. After blowup of $Q$ we gain hyperbolicity. In particular, the purple double-headed arrows in \figref{pws_hysteresis_final} indicate that the direction along the sphere is hyperbolic; this enables the use of center manifold calculations to extend the critical manifold $p=1$, see \secref{entrychartQ}. (I've also added a new subsection to introduce these different arrows, see \secref{notation}.)

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 34 lines 7-10: The sentence ”This gives rise ... transversally”
must be explained in details.
}
\end{enumerate}

\

\textbf{Response:} I've made the sentence simpler. The details are available in \secref{Qblowupvf}.

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 47, line 12: Rewrite the sentence ”In this chart ... manifold.”
}
\end{enumerate}

\

\textbf{Response:} I've modified the text. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 47 line 16: What is the definition of ”canard point” and provide
a proof that it is a canard point following such a definition.
}
\end{enumerate}

\

\textbf{Response:} Good point. I've added references. The text was only in antipication. I believe that this is now clearer in the revised manuscript. The details are summarized in \propref{canard}. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{page 48 Figure 25: I believe that there is a mistake at $0 < \nu_{213,f}$
(maybe $\nu_{213} < \nu_{213,f}$ ). Also, detail the sentence ”The canard ... system”.
}
\end{enumerate}

\

\textbf{Response:} Corrected. Thanks for spotting this. I've change the final sentence in the figure caption regarding the canard. 

\

\begin{enumerate}[resume*=rev1]
	\item \textit{Section 5.4 must be detailed. For example, page 51 line 5: detail the
pages and the number of the theorems where such a results are found in the quoted literature. Also, page 51 line 22: The proof of Theorem 5.1 (2) must
be detailed.
}
\end{enumerate}

\

\textbf{Response:}  I've added more details, including precise references. The verification of the cone properties is identical to \cite[Theorem 4.1]{kristiansen2021a} (see also  \cite[Chapter 14.5]{kuehn2015}). In fact, upon having explained the sets $H_1,\ldots,H_n$ and $V_1,\ldots,V_n$ in full details, the remaining construction is identical to these references (having $n=2$ or $n\ge 2$ makes no difference). I therefore find it to be most appropriate to leave out additional details on this aspect. 
 

\

 \section*{Reviewer \# 2 feedback and reply}

\begin{enumerate}[series=rev2]
	\item \textit{The main criticism I have is that Section 5 (over 20 pages) only goes as far as
essentially recovering the results of [2]. That is, if smoothing dominates we get
a saddle-node bifurcation, while if hysteresis dominates we get chaos. The benefit afforded by system (6) (introduced in [3]) is that it gives both of these in a
single system and so, as written in the concluding section, it would be extremely
interesting “to explore the transition between [these] two regimes”.
Could, over one or two pages, a minimal example system be given and a one-
parameter bifurcation diagram be included showing what bifurcations seem to
occur (at least for this one example) as we go from one regime to the other? How
does chaos arise? No blow-up or hard analysis would be needed, just numerics.
}
\end{enumerate}

\

\textbf{Response:} Thanks for this. I agree that this would be interesting (and this is among the suggestions for future work). However, performing numerical computations on a simple example that addresses this is a highly nontrivial task due to (a) the very singular nature of the problem and (b) due to the fact that the chaos is ``microscopic'' (the horseshoe is exponentially small with respect to $\epsilon,\alpha\rightarrow 0$). 

The fold itself is easy: I have redone the AUTO computations in \cite{2019arXiv190806781U} on the friction oscillator but in the context of \eqref{xypmodel}. I find a fold in agreement with \thmref{main2}, but also for a more wide range of values of $\epsilon$ and $\alpha$. (I've also performed continuation of the fold). However, it is my belief that the transition to chaotic dynamics does not manifest itself directly along the branch of periodic orbits. (The fold most probably coexists with the chaotic dynamics.) We also need to compute the canard and its unstable foliation near $M$. This entails  a substantial amount of work and it is my belief that this is not needed here. 
 For this reason, I have decided not to follow the referee's suggestion. 
 
%  I will also say that  I have redone the AUTO computations in \cite{2019arXiv190806781U} on the friction oscillator but in the context of \eqref{xypmodel}. The calculations are not so easy, due to the very singular nature of the problem, but I find a (single?) fold for a wide range of values of $\epsilon$ and $\alpha$. (I've also performed continuation of the fold). 
% 
% It is my belief that the transition to chaotic dynamics does not manifests itself directly along the branch of periodic orbits. 

I would also like to challenge the argument that the work simply ``recovers the results of [2]''. The work [2] does not study \eqref{xypmodel} but studies regularization by smoothing (see also \cite{2019arXiv190806781U}) and regularization by hysteresis. The present work shows that these distinct results (on two distinct systems) can be unified in the model \eqref{xypmodel} and it is a nontrivial task to do so rigorously. 

% I do, however, provide a short description of what I have done already in the discussion section. 



\

\begin{enumerate}[resume*=rev2]
	\item \textit{Section 3 uses two 2d blow-ups, one in $\alpha$ then one in $\epsilon$. Could Theorem 3.1
instead be proved using one 3d blow-up that does $\alpha$ and $\epsilon$ simultaneously by
writing ($ȳ$, $\alpha$̄, $\epsilon$̄) $\in S^2$. This approach seems simpler to me so I’m guessing there’s
a reason this approach wouldn’t work very well (or at all) otherwise the author
would presumably have used it. Can more explanation be added as to why two
blow-ups are needed?
}
\end{enumerate}

\

\textbf{Response:} By using a single spherical blowup, one is implicitly imposing some order dependency on $y$, $\alpha$ and $\epsilon$. Looking at the term $\phi=\phi\left(\frac{y+\alpha p}{\epsilon\alpha}\right)$ one could be tempted to do
\begin{align*}
 y &= -\alpha p +r^2 \bar y,\\
 \alpha &=r \bar \alpha,\\
 \epsilon &= r\bar \epsilon,
\end{align*}
so that $\phi=\phi(\bar y\bar \epsilon^{-1} \bar \alpha^{-1})$. However, if we look in a chart $(\bar \alpha=1)_1$ then $y+\alpha p=\mathcal O(\alpha^2)$, and $\epsilon = \alpha \epsilon_1$. Similarly, in the chart $(\bar \epsilon=1)_2$ then $y+\alpha p=\mathcal O(\epsilon^2)$ and $\alpha=\epsilon \alpha_2$. In particular, these scalings do not identify $M$ (which is central to the whole construction) unless $\epsilon\sim \alpha$. I have included a short sentence about this at the end of section 2.3.


\

\begin{enumerate}[resume*=rev2]
	\item \textit{
 Sotomeyer and Teixeira 1996 (reference [23]) and others use transition functions
$\phi$ that are constant outside the interval $[−1, 1]$. This contrasts Assumption 2 that
involves decay like $\frac{1}{\vert s\vert^k}$. Given that so much of the calculations in this paper involve
powers of $k$, can the blow-up method still be applied to the transition functions
of [23]? How would the statements of Theorems 3.1 and 5.1 need to be modified
to accommodate them?
}
\end{enumerate}

\

\textbf{Response:} I do not belief that the statements or the approach would change in a signicant way. The constant $k$ just relates to the degree of smoothness of $\phi$ at $s=\pm 1$ (assuming finite smoothness), see \cite[p. 10]{reves_regularization_2014} ($k$ is called $p$ there) and compare \cite[Theorem 2.2]{reves_regularization_2014} with \cite[Theorem 1.3]{2019arXiv190806781U} (the latter using the regularization functions of the present paper). The Sotomayor and Teixeira regularization functions are easier to study because one does not need to compactify; for standard regularizations with $\phi(y\epsilon^{-1})$ being of Sotomayor-Teixeira-type, we can just use $y=\epsilon y_2$ on $y_2\in [-1,1]$ because $\vert y_2\vert>1$ corresponds to $Z_\pm$. I have included short discussion of this following \thmref{main1} and \thmref{main2}.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{
I think it should be stressed that the chaos will not be particularly troubling from
an engineering perspective because the chaotic orbits are all within order-$\alpha$ (or
some power of $\alpha$) of a periodic orbit. Any time-series of the orbit would be almost
oscillatory, just with slightly varying amplitudes at each oscillation. The author
could reference [1] where this is termed ‘micro-chaos’.
}
\end{enumerate}

\

\textbf{Response:} That is a good point. I have followed the advice of the referee and added a reference (see \cite{glendinning2010a}).

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In line 5 of the abstract, I think “becomes smaller” should be “becomes zero”.
}
\end{enumerate}

\

\textbf{Response:} Thanks. Corrected.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{The abstract references [2] and [3]. However, abstracts need to be stand-alone
blocks of text, so references can only be included if their entire bibliographical
details are also included. For this reason I recommend omitting reference to these
papers in the abstract.
}
\end{enumerate}

\

\textbf{Response:} I have removed the references from the abstract as suggested. 

\


\begin{enumerate}[resume*=rev2]
	\item \textit{In Section 1, line 1 of paragraph 2, I think “near $\Sigma$” should be “on $\Sigma$” because
solutions to (1) are well-defined near $\Sigma$.
}
\end{enumerate}

\

\textbf{Response:} Thanks. Corrected.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In Assumption 1, the partial derivatives should be normal derivatives because $\phi$
is a function of just one variable.
}
\end{enumerate}

\

\textbf{Response:} Sure. Corrected.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In line 2 of Assumption 2, I think $[0, \infty]$ should be $[0, \infty)$ because $s$ is a real
number so cannot equal $\infty$.}
\end{enumerate}

\

\textbf{Response:} Thanks. Corrected.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{Just after equation (9), $s = \pm\infty$ should be $s\rightarrow \pm \infty$.
}
\end{enumerate}

\

\textbf{Response:} Thanks. Corrected.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{ In Lemma 1 the third differential equation needs a dot above the p.
}
\end{enumerate}

\

\textbf{Response:} Thanks. In reformulating the Lemma, the equations has been removed. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{  Please refer to Fig. 4 immediately after equation (12) as I think this is where the
reader should look to the figure to get some intuition as to how F behaves.
}
\end{enumerate}

\

\textbf{Response:} Yes, good point. I've followed the advice. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{ Just after equation (16) it says that “by the inverse process the points (x, 0, 0)
are therefore blown up to a cylinder”. But the process is non-invertible if you’re
considering $\epsilon=0$, right? It seems this needs to be reworded.
}
\end{enumerate}

\

\textbf{Response:} By inverse process I meant via the preimage. I have reworded the sentence. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In Proposition 2.1 at the bottom of page 9, what does “coincides on x” mean?
}
\end{enumerate}

\

\textbf{Response:} Good point. I have reworded the sentence. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{On page 10 the reader is given their first taste of a series of charts. Can these
please be explained more? I got confused around the three indented equations
just after “takes the following forms:”. E.g. the first chart has $\bar y= 1$. I thought
$(\bar y,\bar \epsilon)\in S^1$ so doesn’t this mean $\bar \epsilon = 0$ throughout the first chart?
Also just before the next indented equation the $\bar y= −1$ has an unnecessary extra
set of parentheses.
}
\end{enumerate}

\

\textbf{Response:} Yes, this is probably an unfortunate case of ``jargon''. I have included a new section, see \secref{newDirectional} to describe these charts in some generality.  

\

\begin{enumerate}[resume*=rev2]
	\item \textit{Typo just after equation (18): $\epsilon\rightarrow$ is missing $0$.
Also in Section 2.3 “convinient” is spelt wrong twice.
}
\end{enumerate}

\

\textbf{Response:} Thanks. Corrected. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{Figure 12 (also Figure 26) look good on my computer screen, but when I printed
them out they were mostly blank. I’ve no idea why, perhaps an issue with my
printer, and probably not worth worrying about, but perhaps please take a moment
to check to see if there is anything weird with these figures compared to the rest.
}
\end{enumerate}

\

\textbf{Response:} Thanks for this, but I have found nothing wrong with these figures. Hope it looks OK for the referee in the revised version. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In Assumption 5 (and again throughout the rest of Section 5), I think $\mu \sim 0$ should
be $\mu \approx 0$. If not, what exactly does $\mu\sim 0$ mean?
}
\end{enumerate}

\

\textbf{Response:} I've replaced these uses of $\sim$ by $\approx$ as suggested. Please notice that $\sim$ is used in a different way in \secref{main2}, see \eqref{sim} and the explaination below this equation. 

\

\begin{enumerate}[resume*=rev2]
	\item \textit{Last line of page 31 and first line of page 32: “Then upon using [1]”. This is
unclear. Are you using a particular mathematical result that was proved in [1]?
}
\end{enumerate}

\

\textbf{Response:} Good point. This has now been corrected with a reference to \cite[Proposition 14]{reves_regularization_2014}.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{ Regarding Theorem 5.1, please explain a bit about what “a full shift on n symbols”
means and how it represents chaos (e.g. sensitive dependence on initial conditions).
It seems remarkable that the results gives any possible value for n, because often
one just does $n = 2$ I think.
}
\end{enumerate}

\

\textbf{Response:} Good point. I have added some explaination and included \propref{shift}.

\

\begin{enumerate}[resume*=rev2]
	\item \textit{In line 2 of Section 6 the statement that the analysis is just done for $\alpha > 0$ feels
weak. I think here you should remind the reader that $\alpha > 0$ corresponds to normal
hysteresis (i.e. feedback) so this is more important to treat than $\alpha < 0$.
}
\end{enumerate}

\

\textbf{Response:} Good point. I have followed the advice of the referee.

\

